Data Certification Strategies for Blockchain-based Traceability Systems

The use of blockchains for data certification and traceability is now well established in both the literature and practical applications. However, while blockchain-based certification of individual data is clear and straightforward, the use of blockchain to certify large amounts of data produced on a nearly continuous basis still poses some challenges. In such a case, in fact, it is first necessary to collect the data in an off-chain buffer, and then to organize it, e.g., via Merkle trees, in order to keep the size and quantity of certification data to be written to the blockchain small. In this paper, we consider a typical system for blockchain-based traceability of a production process, and propose and comparatively analyze some strategies for certifying the data of such a process on blockchain, while maintaining the possibility of verifying their certification in a decentralized way.

==> imgs/comp_cost.tex <==
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}
  \begin{axis}[
xtick={128,512,1024,2048},   
%xticklabels={0,0.25$\textcolor{white}{2^8}$,0.5,0.75,1},   
%ytick={1,0.1,0.01,0.001,0.0001,0.00001,0.000001,0.0000001},
xmin = 128,
xmax= 2048,
grid = both,
ymin=0,
ymax=1500,
%ymode = log,
legend style={at={(0.5,0.97)},anchor=north},
mark size=2pt,
xlabel={Data entries},
ylabel={Transaction cost [€]},
xticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
}]

\addplot[red, line width=1pt]coordinates{

(128, 83.2)
(512, 332.8)
(1024, 665.6)
(2048, 1331.2)
};\addlegendentry{Single data};

\addplot[blue, line width=1pt]coordinates{

(128, 0.6)
(512, 0.6)
(1024, 0.6)
(2048, 0.6)
};\addlegendentry{Multiple data};

 
\end{axis}
\end{tikzpicture}}

==> imgs/comp_storage.tex <==
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}
  \begin{axis}[
xtick={128,512,1024,2048},   
%xticklabels={0,0.25$\textcolor{white}{2^8}$,0.5,0.75,1},   
%ytick={0,1, 10, 100, 1000},
xmin = 128,
xmax= 2048,
grid = both,
ymin=0,
ymax=150,
%ymode = log,
legend style={at={(0.5,0.97)},anchor=north},
mark size=2pt,
xlabel={Data entries},
ylabel={Storage [kB]},
xticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
}]

\addplot[red, line width=1pt]coordinates{

(128, 0.00001)
(512, 0.00001)
(1024, 0.00001)
(2048, 0.00001)
};\addlegendentry{Single data};

\addplot[blue, line width=1pt]coordinates{

(128, 7.7)
(512, 32.3)
(1024, 65)
(2048, 130.6)
};\addlegendentry{Multiple data};

 
\end{axis}
\end{tikzpicture}}

==> imgs/comp_verif.tex <==
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}
  \begin{axis}[
xtick={128,512,1024,2048},   
%xticklabels={0,0.25$\textcolor{white}{2^8}$,0.5,0.75,1},   
%ytick={0,1, 10, 100, 1000},
xmin = 128,
xmax= 2048,
grid = both,
ymin=0,
ymax=20,
%ymode = log,
legend style={at={(0.5,0.03)},anchor=south},
mark size=2pt,
xlabel={Data entries},
ylabel={Execution time [ms]},
xticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=5
}]

\addplot[red, line width=1pt]coordinates{

(128, 13)
(512, 13)
(1024, 13)
(2048, 13)
};\addlegendentry{Single data};

\addplot[blue, line width=1pt]coordinates{

(128, 16)
(512, 17)
(1024, 17)
(2048, 18)
};\addlegendentry{Multiple data};

 
\end{axis}
\end{tikzpicture}}
